Higgs oscillations in a unitary Fermi superfluid

Symmetry-breaking phase transitions are central to our understanding of states of matter. When a continuous symmetry is spontaneously broken, new excitations appear that are tied to fluctuations of the order parameter. In superconductors and fermionic superfluids, the phase and amplitude can fluctuate independently, giving rise to two distinct collective branches. However, amplitude fluctuations are difficult to both generate and measure, as they do not couple directly to the density of fermions and have only been observed indirectly to date. Here, we excite amplitude oscillations in an atomic Fermi gas with resonant interactions by an interaction quench. Exploiting the sensitivity of Bragg spectroscopy to the amplitude of the order parameter, we measure the time-resolved response of the atom cloud, directly revealing amplitude oscillations at twice the frequency of the gap. The magnitude of the oscillatory response shows a strong temperature dependence, and the oscillations appear to decay faster than predicted by time-dependent BCS theory applied to our experimental setup.

==> config.tex <==

%Packages

\usepackage[utf8]{inputenc}
\usepackage{amsmath, amssymb, amsthm}
\usepackage{graphicx}
%\usepackage{subcaption}
\usepackage{sidecap}
%\usepackage{textcomp}
\usepackage{tikz}
\usetikzlibrary{patterns}
\usepackage{xcolor}
%\usepackage{pgfplots}
\usepackage{braket}
\usepackage{tabularx}
\usepackage{color,colortbl}
\usepackage{appendix}
%\usepackage{cite}
\usepackage{hyperref}
\usepackage{url}
\usepackage{mathtools}
\usepackage{bigints}
\usepackage{relsize}
\usepackage[thinlines]{easytable}
%\usepackage[numbers, sort&compress]{natbib}
%\usepackage{natbib}
%\usepackage[font=small,labelfont=bf]{caption}
%\captionsetup{justification=justified,singlelinecheck=false}
\usepackage[a4paper,width=150mm,top=30mm,bottom=30mm, bindingoffset=6mm]{geometry}
\usepackage{pgfplots}
\usepackage{siunitx}


%Extra commands
\newcommand{\pg}{\mathbf{p}}
\newcommand{\qg}{\mathbf{q}}
\newcommand{\rg}{\mathbf{r}}
\newcommand{\kg}{\mathbf{k}}
\newcommand{\xg}{\mathbf{x}}
\newcommand{\Qg}{\mathbf{Q}}
\newcommand{\psih}{\hat{\psi}}
\newcommand{\ha}{\hat{a}}
\newcommand{\had}{\hat{a}^\dagger}
\newcommand{\up}{\uparrow}
\newcommand{\down}{\downarrow}
\newcommand{\bint}{\mathlarger{\mathlarger{‎‎\int}}}
\newcommand{\bsum}{\mathlarger{\mathlarger{‎‎\sum}}}
\newcommand{\aprime}{'}
\newcommand{\apx}{''}
\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\qte}[1]{\textquotedblleft{#1}\textquotedblright}



\usepackage{soul}
\definecolor{viola}{rgb}{0.54, 0.17, 0.89}
\newcommand{\viol}[1]{{\color{viola} #1 }}

%Hadrien's commands

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bmul}{\begin{multline}}
\newcommand{\emul}{\end{multline}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\rr}{\mathbf{r}}
\newcommand{\kk}{\mathbf{k}}
\newcommand{\qq}{\mathbf{q}}
\newcommand{\KK}{\mathbf{K}}
\newcommand{\QQ}{\mathbf{Q}}
\newcommand{\pp}{\mathbf{p}}
\newcommand{\lr}{\mathbf{l}}
\newcommand{\zero}{\mathbf{0}}

\newcommand{\ii}{\mathrm{i}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\eee}{\mathrm{e}}

\newcommand{\meanv}[1]{\langle #1 \rangle}
\newcommand{\meanvl}[1]{\overline{#1}}
\newcommand{\meanvlr}[1]{\left\langle #1 \right\rangle}


\newcommand{\comm}[2]{\left[ #1,#2 \right]}
\newcommand{\Tr}[1]{\text{Tr} \bb{#1}}
\newcommand{\g}[1]{«~#1~»}


\newcommand{\bb}[1]{\left( #1 \right)}
\newcommand{\bbr}[1]{\left. #1 \right)}
\newcommand{\bbl}[1]{\left( #1 \right.}
\newcommand{\bbcro}[1]{\left[ #1 \right]}
\newcommand{\bbcror}[1]{\left. #1 \right]}
\newcommand{\bbcrol}[1]{\left[ #1 \right.}
\newcommand{\bbaco}[1]{\left\{ #1 \right\}}
\newcommand{\bbacol}[1]{\left\{ #1 \right.}
\newcommand{\bbacor}[1]{\left. #1 \right\}}
\newcommand{\bbv}[1]{\left\vert #1 \right\vert}
\newcommand{\eval}[1]{\left. #1 \right|}

